A Survey Of Model Fits to Brown Dwarf Spectra Through the L-T Sequence

We fit archival near-infrared spectra of 305 brown dwarfs with atmosphere models from the Sonora and Phoenix groups. Using the parameters of the best-fit models as estimates for the physical properties of the brown dwarfs in our sample, we have performed a survey of how brown dwarf atmospheres evolve with spectral type and temperature. We present the fit results and observed trends. We find that clouds have a more significant impact on near infrared spectra than disequilibrium chemistry, and that silicate clouds influence the near infrared spectrum through the late T types. We note where current atmosphere models are able to replicate the data and where the models and data conflict. We also categorize objects with similar spectral morphologies into families and discuss possible causes for their unique spectral traits. We identify two spectral families with morphologies that are likely indicative of binarity.

==> table9.tex <==
\begin{document}

\startlongtable
\begin{deluxetable}{ccccccccccc}
\tabletypesize{\footnotesize}
\label{tab:speXData}

%% Rotate to a landscape orientation
\tablecaption{Archival Data}
\tablehead{\colhead{Object} & \colhead{OType} & \colhead{IRType} & \colhead{2MASS J} & \colhead{2MASS H} & \colhead{2MASS Ks} & \colhead{Parallax} & \colhead{Sources} \\ 
\colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} } 

%% All data must appear between the \startdata and \enddata commands
\startdata
SDSS J000013.54+255418.6  &  T5  &  T4.5  & 15.063 & 14.731 & 14.836 & 70.8 & 66,9,9,26 \\
SDSS J000250.98+245413.8  &  ----  &  L5.5  & 17.165 & 16.06 & 15.656 &  ----  & 18,18 \\
LHS 102B (J00043484-4044058)  &  L5  &  L4.5  & 13.109 & 12.055 & 11.396 & 82.346602 & 45,50,17,35 \\
2MASS J00150206+2959323  &  L7  &  L7.5pec (blue)  & 16.158 & 15.226 & 14.482 & 31.6 & 47,47,47,4 \\
2MASS J00165953-4056541  &  L3.5  &  L4.5:  & 15.32 & 14.206 & 13.432 & 28.823598 & 46,13,13,35 \\
2MASS J00193927-3724392  &  L3:  &  L2.2 INT-G  & 15.52 & 14.47 & 13.689 & 25.008017 & 13,33,13,35 \\
2MASS J0028208+224905  &  ----  & L6 & 15.607 & 14.468 & 13.781 & 42.8879 & 82,13,35 \\
2MASSW J0030300-145033  &  L7  &  L6:FLD-G  & 16.278 & 15.273 & 14.481 & 41.1 & 44,55,13,4 \\
SDSSp J003259.36+141036.6  &  ----  &  L9  & 16.83 & 15.648 & 14.946 & 30.14 & 62,13,29 \\
2MASS J00345157+0523050  &  ----  &  T6.5  & 15.535 & 15.443 & 16.243 & 105.4 & 9,14,29 \\
2MASSW J0036159+182110  &  L3.5  &  L4:  & 12.466 & 11.588 & 11.058 & 114.473464 & 44,50,15,35 \\
SDSS J003609.26+241343.3  &  ----  &  L5.5  & 17.033 & 16.108 & 15.657 &  ----  & 18,18 \\
HD 3651B (J0039191+211516)  &  ----  &  T7.5  & 16.595 & 16.661 & 16.734 & 90.03 & 59,17,29 \\
2MASS J00501994-3322402  &  ----  &  T7  & 15.928 & 15.838 & 15.241 & 94.6 & 9,9,76 \\
2MASSW J0051107-154417  &  L3.5  &  L5:  & 15.28 & 14.164 & 13.466 & 29.812932 & 44,13,13,35 \\
2MASS J00531899-3631102  &  L3.5  &  L4:  & 14.445 & 13.48 & 12.937 & 40.198959 & 46,61,13,35 \\
2MASSI J0103320+193536  &  L6 beta  &  L6:INT-G  & 16.288 & 14.897 & 14.149 & 46.9 & 29,2,19,29 \\
SDSSp J010752.33+004156.1  &  L8  &  L5.5  & 15.824 & 14.512 & 13.709 & 64.13 & 42,60,13,29 \\
2MASSI J0117474-340325  &  L1 beta  &  L1:INT-G  & 15.178 & 14.209 & 13.489 & 25.39701 & 31,2,15,35 \\
SDSS J011912.22+240331.6  &  ----  &  T2  & 17.017 & 15.953 & 17.042 & 28.9 & 18,18,4 \\
2MASS J01311838+3801554  &  L4:  &  L1.5  & 14.679 & 13.696 & 13.054 & 40.923542 & 21,13,13,35 \\
2MASS J01340281+0508125  &  ----  &  L1  & 16.19 & 15.163 & 14.634 &  ----  & 47,47 \\
IPMS J013656.57+093347.3  &  T2  &  T2.5  & 13.455 & 12.771 & 12.562 & 163.447846 & 66,60,15,35 \\
2MASS J01414839-1601196  &  ----  &  L7:  & 16.209 & 15.161 & 14.344 & 28.8 & 47,47,4 \\
2MASS J01415823-4633574  &  L0 gamma  &  L0: VL-G  & 14.83 & 13.875 & 13.1 & 27.288053 & 22,2,49,35 \\
2MASS J01443536-0716142  &  L5  &  L5  & 14.191 & 13.008 & 12.268 & 78.497841 & 51,61,15,35 \\
2MASS J01472702+4731142  &  ----  &  L1.5  & 15.843 & 14.847 & 14.282 & 20.8459 & 47,47,35 \\
SDSS J015141.69+124429.6  &  ----  &  T1  & 16.566 & 15.603 & 15.183 & 46.73 & 9,14,29 \\
2MASS J01550354+0950003  &  L5  &  L3.2 INT-G  & 14.825 & 13.763 & 13.139 & 45.042214 & 68,33,23,35 \\
SDSS J020735.60+135556.3  &  L3  &  L3:  & 15.462 & 14.474 & 13.808 & 26.688561 & 42,50,9,35 \\
2MASSW J0205034+125142  &  L5  &  L5.5  & 15.679 & 14.449 & 13.671 & 42.5 & 44,13,67,4 \\
DENIS-P J0205.4-1159  &  L7  &  L5.5::  & 14.587 & 13.568 & 12.998 & 49.346327 & 48,50,13,35 \\
2MASS J02055138-0759253  &  L3  &  L2  & 16.031 & 15.169 & 14.358 &  ----  & 69,47,47 \\
SDSS J020608.97+223559.2  &  ----  &  L4.5 blue  & 16.556 & 15.538 & 15.162 &  ----  & 70,18 \\
SDSS J020742.48+000056.2  &  ----  &  T4.5  & 16.799 & 16.396 & 15.412 & 34.85 & 9,9,29 \\
2MASSW J0208236+273740  &  L5  &  L5  & 15.714 & 14.56 & 13.872 & 21.3 & 44,13,13,4 \\
2MASSW J0208183+254253  &  L1  &  ----  & 13.989 & 13.107 & 12.588 & 43.09921 & 44,15,35 \\
2MASS J02271036-1624479  &  L1  &  L0.5:  & 13.573 & 12.63 & 12.143 & 49.8637799 & 68,61,15,35 \\
2MASSW J0228110+253738  &  L0:  &  L0  & 13.839 & 12.993 & 12.471 & 28.7 & 20,79,15,4 \\
2MASS J02304442-3027275  &  ----  &  L1  & 15.822 & 15.21 & 14.886 & 17.37149 & 47,47,35 \\
GJ 1048B (J02355993-2331205)  &  L1  &  L1  & 12.69 & 12.725 & 12.186 & 46.417968 & 40,40,15,35 \\
2MASSI J0241536-124106  &  L2:  &  L1.9  & 15.605 & 14.646 & 13.931 & 25.419938 & 20,3,15,35 \\
SDSS J024256.98+212319.6  &  ----  &  L4  & 16.977 & 15.938 & 15.474 &  ----  & 18,18 \\
2MASSI J0243137-245329  &  T5.5  &  T6  & 15.381 & 15.137 & 15.216 & 93.46 & 66,9,14,26 \\
SDSS J024749.90-163112.6  &  ----  &  T2:  & 17.186 & 16.17 & 15.616 &  ----  & 18,18 \\
DENIS-P J0255-4700  &  L8  &  L9  & 13.246 & 12.204 & 11.558 & 205.425085 & 46,9,9,35 \\
2MASS J02572581-3105523  &  L8  &  L8:  & 14.672 & 13.518 & 12.876 & 102.69926 & 46,61,72,35 \\
2MASS J03001631+2130205  &  ----  &  L6 pec (sl. Blue)  & 15.921 & 14.885 & 14.258 &  ----  & 47,47 \\
2MASSW J0310599+164816  &  L8  &  L9  & 16.025 & 14.932 & 14.312 & 36.9 & 44,9,17,77 \\
2MASS J03185403-3421292  &  L7  &  L6.5  & 15.569 & 14.346 & 13.507 & 70.98123 & 46,13,13,35 \\
2MASSW J0320284-044636  &  M8  &  L0.5  & 13.259 & 12.535 & 12.134 & 47.602063 & 20,79,15,35 \\
SDSS J032553.17+042540.1  &  ----  &  T5.5  & 16.25 & 16.08 & 16.525 & 44 & 18,18,4 \\
2MASSI J0328426+230205  &  L8  &  L9.5  & 16.693 & 15.547 & 14.916 & 33.13 & 44,50,15,29 \\
2MASP J0345432+254023  &  L0  &  L1:  & 13.997 & 13.211 & 12.672 & 37.894834 & 48,50,6,35 \\
SDSS J035104.37+481046.8  &  ----  &  T1:  & 16.466 & 15.566 & 14.996 & 28.5 & 18,18,4 \\
2MASS J04070752+1546457  &  L3.5  &  L3:FLD-G  & 15.478 & 14.354 & 13.559 & 28.280145 & 68,2,15,35 \\
2MASS J04070885+1514565  &  ----  &  T5  & 16.055 & 16.017 & 15.922 & 55.4 & 9,14,4 \\
2MASS J04062677-3812102  &  L0gamma  &  L1:VL-G  & 16.756 & 15.624 & 15.111 &  ----  & 47,2,47 \\
2MASSI J0415195-093506  &  T8  &  T8  & 15.695 & 15.537 & 15.429 & 174.34 & 8,9,14,35 \\
SDSSp J042348.57-041403.5  &  L7.5  &  T0  & 14.465 & 13.463 & 12.929 & 70.150173 & 20,9,14,35 \\
2MASSI J0439010-235308  &  L6.5  &  L6  & 14.408 & 13.409 & 12.816 & 80.726633 & 20,13,17,35 \\
2MASS J0447430-193604  &  L5:  &  ----  & 15.969 & 14.785 & 14.012 & 20.7 & 13,13,4 \\
2MASS J05103520-4208140  &  ----  &  T5  & 16.222 & 16.237 & 15.996 &  & 56,56 \\
2MASS J05160945-0445499  &  ----  &  T5.5  & 15.984 & 15.721 & 15.486 & 54.2 & 9,15,4 \\
2MASS J05161597-3332046  &  L3:  &  L4.5:  & 15.879 & 14.801 & 13.987 &  ----  & 13,13,13 \\
2MASS J05185995-2828372  &  L7  &  T1p  & 15.978 & 14.83 & 14.162 & 47.5 & 46,9,19,29 \\
SDSSp J053951.99-005902.0  &  L5  &  L5  & 14.033 & 13.104 & 12.527 & 78.945088 & 32,50,24,35 \\
2MASS J05591914-1404488  &  T5  &  T4.5  & 13.802 & 13.679 & 13.577 & 95.271437 & 8,9,9,35 \\
2MASS J06020638+4043588  &  ----  &  T4.5  & 15.544 & 15.592 & 15.166 & 65.1 & 56,56,4 \\
2MASS J06244595-4521548  &  L5:  &  L6  & 14.48 & 13.335 & 12.595 & 82.024763 & 68,61,72,35 \\
2MASSI J0652307+471034  &  L4.5  &  L6.5  & 13.511 & 12.384 & 11.694 & 109.765056 & 20,13,13,35 \\
SDSS J065405.63+652805.4  &  ----  &  L6:  & 16.138 & 15.196 & 14.603 &  ----  & 18,13 \\
2MASSW J0717163+570543  &  L3  &  L6.5  & 14.636 & 13.593 & 12.945 & 34.547104 & 68,79,13,35 \\
2MASSI J0727182+171001  &  T8  &  T7  & 15.6 & 15.756 & 15.556 & 110.14 & 8,9,9,29 \\
2MASS J07290002-3954043  &  ----  &  T8pec  & 15.92 & 15.979 & 15.29 & 126.3 & 56,56,29 \\
SDSS J073922.26+661503.5  &  ----  &  T1.5:  & 16.823 & 15.998 & 15.831 &  ----  & 18,13 \\
SDSS J074149.15+235127.5  &  ----  &  T5  & 16.158 & 15.838 & 15.847 & 53 & 9,13,4 \\
2MASS J07415784+0531568  &  ----  &  L1.5  & 14.379 & 13.563 & 13.062 & 38.35271 & 47,47,35 \\
SDSS J074201.41+205520.5  &  ----  &  T5  & 16.193 & 15.911 & 15.225 & 58.4 & 9,13,4 \\
2MASSI J0755480+221218  &  T6  &  T5  & 15.728 & 15.669 & 15.753 & 58.9 & 8,9,9,4 \\
SDSS J075840.33+324723.4  &  T3  &  T2  & 14.947 & 14.111 & 13.879 & 93.7 & 66,9,15,4 \\
2MASSW J0801405+462850  &  L6.5  &  L5.5  & 16.275 & 15.452 & 14.536 &  ----  & 44,13,13 \\
SDSS J080531.84+481233.0  &  L4  &  L9:  & 14.734 & 13.917 & 13.444 & 42.594613 & 42,50,17,35 \\
2MASSW J0820299+450031  &  L5  &  L4.5::  & 16.279 & 15 & 14.218 & 30.9 & 44,13,13,4 \\
SDSS J082030.12+103737.0  &  ----  &  L9.5::  & 16.98 & 16.079 & 15.538 &  ----  & 18,18 \\
2MASS J08234818+2428577  &  L3  &  L1.5  & 14.986 & 14.06 & 13.377 & 40.108827 & 68,13,13,35 \\
2MASSI J0825196+211552  &  L7.5  &  L6  & 15.1 & 13.792 & 13.028 & 92.600579 & 44,60,13,35 \\
SSSPM 0829-1309  &  L2  &  ----  & 12.803 & 11.851 & 11.297 & 85.6014 & 83,17,35 \\
SDSSp J083008.12+482847.4  &  L8  &  L9:  & 15.444 & 14.343 & 13.676 & 80.6289 & 46,37,15,35 \\
SDSS J083048.80+012831.1  &  ----  &  T4.5  & 16.289 & 16.14 & 16.358 & 42.7 & 9,13,4 \\
SDSS J083506.16+195304.4  &  ----  &  L4.5  & 16.094 & 14.889 & 14.319 &  ----  & 18,18 \\
2MASSI J0835425-081923  &  L5  &  L4 pec  & 13.169 & 11.938 & 11.136 & 138.314729 & 20,33,13,35 \\
SDSSp J083717.22-000018.3  &  T0  &  T1  & 17.101 & 15.988 & 15.674 & 29.8 & 46,9,9,4 \\
2MASSI J0847287-153237  &  L2  &  ----  & 13.513 & 12.629 & 12.061 & 57.510617 & 20,63,35 \\
2MASSs J0850359+105716  &  L6  &  ----  & 16.465 & 15.221 & 14.473 & 31.4 & 48,16,27 \\
SDSS J085116.20+181730.0  &  ----  &  L4.4 FLD-G  & 16.567 & 15.948 & 14.968 &  ----  & 33,18 \\
SDSS J085234.90+472035.0  &  ----  &  L9.5:  & 16.182 & 15.419 & 14.718 & 42.2 & 50,13,4 \\
2MASSI J0856479+223518  &  L3:  &  ----  & 15.679 & 14.58 & 13.951 & 31.810112 & 20,13,35 \\
SDSSp J085758.45+570851.4  &  L8  &  L8:  & 15.038 & 13.79 & 12.962 & 72.719722 & 46,37,13,35 \\
SDSS J085834.42+325627.7  &  ----  &  T1  & 16.453 & 15.382 & 14.756 & 40.9 & 18,13,4 \\
2MASS J09054654+5623117  &  L5  &  L6  & 15.395 & 14.284 & 13.73 & 41.295777 & 68,13,13,35 \\
2MASSI J0908380+503208  &  L5  &  L9:  & 14.549 & 13.477 & 12.945 & 95.92903 & 20,50,72,35 \\
SDSS J090900.73+652527.2  &  T1  &  T1.5  & 16.034 & 15.214 & 15.171 &  ----  & 60,18,18 \\
Gl 337CD (J09121469+1459396)  &  L8  &  T0  & 15.512 & 14.621 & 14.043 & 46.4 & 78,9,13,4 \\
2MASS J09153413+0422045  &  L6  &  ----  & 14.548 & 13.531 & 13.011 & 59.9 & 68,17,4 \\
2MASSW J0920122+351742  &  L6.5  &  T0p  & 15.625 & 14.673 & 13.979 & 34.4 & 44,9,13,26 \\
2MASS J09211410-2104446  &  L1.5  &  L4:  & 12.779 & 12.152 & 11.69 & 79.572926 & 68,11,17,35 \\
SDSSp J092615.38+584720.9  &  T5  &  T4.5  & 15.897 & 15.307 & 15.45 & 43.7 & 66,9,13,26 \\
2MASSW J0929336+342952  &  L8  &  L7.5  & 16.601 & 15.44 & 14.644 &  ----  & 44,50,13 \\
2MASSI J0937347+293142  &  T7  &  T6p  & 14.648 & 14.703 & 15.267 & 163.39 & 8,9,9,29 \\
2MASS J09393548-2448279  &  T8  &  T8  & 15.98 & 15.797 & 16.556 & 196 & 66,9,9,29 \\
2MASS J09490860-1545485  &  ----  &  T2  & 16.149 & 15.262 & 15.227 & 32.9 & 9,9,4 \\
SDSS J100711.74+193056.2  &  ----  &  L8:  & 16.871 & 15.755 & 14.997 & 45.6 & 18,13,4 \\
2MASS J10073369-4555147  &  ----  &  T5  & 15.653 & 15.686 & 15.56 & 71 & 56,56,29 \\
2MASSI J1010148-040649  &  L6  &  L6  & 15.508 & 14.385 & 13.619 & 55 & 20,47,67,4 \\
SDSS J102109.69-030420.1  &  T3.5  &  T3  & 16.253 & 15.346 & 15.126 & 33.7 & 46,9,9,27 \\
HD 89744B (J10221489+4114266)  &  L0  &  & 14.901 & 14.022 & 13.608 & 26.007036 & 78,15,35 \\
SDSS J102552.43+321234.0  &  ----  &  L7:FLD-G  & 15.913 & 15.593 & 15.072 & 37.3 & 55,18,55 \\
SDSS J103026.78+021306.4  &  ----  &  L9.5:  & 16.889 & 16.175 & 15.079 & 19.5 & 50,13,4 \\
2MASS J10315064+3349595  &  ----  &  L2  & 15.923 & 14.838 & 14.364 & 21.5184 & 47,47,35 \\
SDSS J103321.92+400549.5  &  ----  &  L6  & 16.644 & 15.874 & 15.408 &  ----  & 18,18 \\
2MASSW J1036530-344138  &  L6  &  L6.5  & 15.622 & 14.446 & 13.798 & 67.960842 & 41,13,13,35 \\
SDSS J103931.35+325625.5  &  ----  &  T1  & 16.405 & 15.335 & 15.151 & 30 & 18,13,4 \\
2MASS J10430758+2225236  &  L8  &  L9:  & 15.965 & 14.725 & 13.991 & 52.4 & 20,13,72,4 \\
SDSS J104335.08+121314.1  &  ----  &  L9  & 15.997 & 14.969 & 14.258 & 59.9 & 47,47,4 \\
SDSS J104409.43+042937.6  &  ----  &  L7  & 15.881 & 14.95 & 14.259 & 30.8 & 50,13,4 \\
2MASSI J1047538+212423  &  T7  &  T6.5  & 15.819 & 15.797 & 16.408 & 94.73 & 8,9,15,29 \\
SDSS J104842.84+011158.5  &  L1  &  L4  & 12.924 & 12.14 & 11.623 & 66.589368 & 42,43,15,35 \\
2MASS J10461875+4441149  &  ----  &  L5 pec (sl. Blue)  & 15.622 & 14.656 & 14.13 & 28.903592 & 47,47,35 \\
SDSS J104829.21+091937.8  &  ----  &  T2.5  & 16.594 & 15.898 & 16.365 &  ----  & 18,13 \\
SDSS J105213.51+442255.7  &  L7.5  &  T0.5:  & 15.958 & 15.161 & 14.568 &  ----  & 66,18,15 \\
DENIS-P J1058.7-1548  &  L3  &  L2.2 FLD-G  & 14.155 & 13.226 & 12.532 & 55.098508 & 48,33,13,35 \\
2MASS J10595185+3042059  &  ----  &  T4  & 16.195 & 15.766 & 15.56 & 38.6 & 71,71,4 \\
2MASS J11000965+4957470  &  L3.5  &  L3  & 15.282 & 14.192 & 13.474 & 39.27727 & 68,13,72,35 \\
2MASSI J1104012+195921  &  L4  &  L5.5  & 14.38 & 13.476 & 12.95 & 55.704629 & 20,13,14,35 \\
SDSSp J111010.01+011613.1  &  ----  &  T5.5  & 16.343 & 15.924 & 15.129 & 52.1 & 9,9,76 \\
Gliese 417BC (J11122567+3548131)  &  L4.5  &  L5:FLD-G  & 14.584 & 13.499 & 12.721 & 42.244704 & 44,2,13,35 \\
SDSS J111320.16+343057.9  &  ----  &  L3  & 16.767 & 15.803 & 15.51 &  ----  & 18,18 \\
2MASS J11145133-2618235  &  T8  &  T7.5  & 15.858 & 15.734 & 16.109 & 176.8 & 66,9,9,29 \\
2MASS J11181292-0856106  &  L6  &  L6 pec (blue)  & 15.784 & 14.731 & 14.296 & 43.6501 & 47,47,47,35 \\
SDSS J112118.57+433246.5  &  ----  &  L7.5  & 17.006 & 16.231 & 15.572 &  ----  & 18,18 \\
2MASS J11220826-3512363  &  ----  &  T2  & 15.019 & 14.358 & 14.383 & 75.437994 & 9,9,35 \\
2MASS J11263991-5003550  &  L4.5  &  L6.5:: pec  & 13.997 & 13.284 & 12.829 & 61.833073 & 11,11,15,35 \\
2MASSW J1146345+223053  &  L3  &  ----  & 14.165 & 13.182 & 12.59 & 36.8 & 48,13,29 \\
SDSS J115553.86+055957.5  &  ----  &  L6.8 FLD-G  & 15.66 & 14.703 & 14.118 & 46.5 & 33,13,4 \\
2MASS J11582077+0435014  &  sdL7  &  sdL7  & 15.611 & 14.684 & 14.439 & 37.3166 & 47,47,47,35 \\
2MASS J12070374-3151298  &  L3:  &  L2.5  & 15.85 & 14.719 & 13.997 & 28.230211 & 68,13,72,35 \\
SDSS J120602.51+281328.7  &  ----  &  T3  & 16.541 & 15.815 & 15.817 & 34 & 18,18,4 \\
SDSS J120747.17+024424.8  &  L8  &  T0  & 15.58 & 14.561 & 13.986 & 44.8 & 42,9,56,4 \\
2MASS J12095613-1004008  &  T3.5  &  T3  & 15.914 & 15.329 & 15.062 & 47.3 & 46,9,14,29 \\
2MASS J12154432-3420591  &  ----  &  T4.5  & 16.236 & 15.809 & 16.317 & 39.8 & 56,56,29 \\
SDSS J121440.95+631643.4  &  ----  &  T3.5:  & 16.586 & 15.779 & 15.877 &  ----  & 18,18 \\
SDSS J121659.17+300306.3  &  ----  &  L3.5:  & 17.072 & 15.739 & 15.813 &  ----  & 18,18 \\
2MASSI J1217110-031113  &  T7  &  T7.5  & 15.86 & 15.748 & 15.887 & 90.8 & 8,9,9,29 \\
SDSS J121951.45+312849.4  &  ----  &  L8  & 15.913 & 14.907 & 14.305 & 52 & 18,13,4 \\
2MASS J12212770+0257198  &  L0  &  M9.7 FLD-G  & 13.169 & 12.41 & 11.953 & 53.811865 & 68,33,15,35 \\
2MASS J12255432-2739466  &  T6  &  T6  & 15.26 & 15.098 & 15.073 & 75.1 & 8,7,14,29 \\
DENIS-P J1228.2-1547  &  L5  &  L6::  & 14.378 & 13.347 & 12.767 & 134.4 & 48,50,13,26 \\
2MASS J12304562+2827583  &  ----  &  L4:  & 16.073 & 15.005 & 14.434 & 22.873855 & 47,71,35 \\
2MASS J12314753+0847331  &  T6  &  T5.5  & 15.57 & 15.309 & 15.22 & 70.2 & 66,9,14,4 \\
2MASS J12373919+6526148  &  T7  &  T6.5  & 16.053 & 15.739 & 16.058 & 96.07 & 8,9,53,29 \\
2MASSW J1239272+551537  &  L5  &  ----  & 14.711 & 13.568 & 12.792 & 42.4 & 44,13,26 \\
2MASS J12474944-1117551  &  ----  &  L0:  & 15.991 & 15.104 & 14.725 &  ----  & 47,47 \\
SDSSp J125453.90-012247.4  &  T2  &  T2  & 14.891 & 14.09 & 13.837 & 74.183846 & 8,9,14,34 \\
2MASS J13023811+5650212  &  L2  &  L3:pec(sl. Blue)  & 16.36 & 15.469 & 14.972 &  ----  & 47,47,47 \\
Kelu-1 (J13054019-2541059)  &  L2  &  L0.5 pec  & 13.414 & 12.392 & 11.747 & 49.045944 & 48,81,17,35 \\
2MASS J13184794+1736117  &  ----  &  L5.5  & 16.341 & 15.227 & 14.533 &  ----  & 47,47 \\
2MASS J13243553+6358281  &  ----  &  T2.5 pec  & 15.596 & 14.576 & 14.058 &  ----  & 47,56 \\
SDSSp J132629.82-003831.5  &  L8:  &  L7  & 16.103 & 15.05 & 14.208 & 47.9 & 32,62,13,4 \\
2MASS J13313310+3407583  &  L0  &  L10: FLD-G  & 14.168 & 13.333 & 12.868 & 34.790813 & 68,55,47,35 \\
SDSS J133148.92-011651.4  &  L6  &  L6:  & 15.459 & 14.475 & 14.073 & 47.1264 & 42,62,13,35 \\
SDSS J134203.11+134022.2  &  ----  &  L5.5  & 16.756 & 15.708 & 15.109 &  ----  & 18,18 \\
SDSS J134525.57+521634.0  &  ----  &  L3.5  & 16.945 & 16.257 & 15.348 &  ----  & 18,18 \\
SDSSp J134646.45-003150.4  &  T7  &  T6.5  & 16 & 15.459 & 15.772 & 68.3 & 8,9,9,29 \\
2MASS J13571237+1428398  &  L3  &  L3:  & 15.584 & 14.647 & 13.88 &  ----  & 69,13,13 \\
SDSS J135852.68+374711.9  &  ----  &  T4.5:  & 16.46 & 16.142 & 16.099 & 49.6 & 18,18,4 \\
SDSS J140023.12+433822.3  &  ----  &  L7:  & 16.301 & 15.094 & 14.487 & 40.8 & 18,13,4 \\
2MASS J14044941-3159329  &  T0  &  T2.5  & 15.577 & 14.955 & 14.538 & 42.5 & 57,56,56,27 \\
2MASS J14075361+1241099  &  L1::  &  L5  & 15.378 & 14.344 & 13.598 & 35.202138 & 68,13,13,35 \\
2MASS J14162409+1348267  &  L6  &  ----  & 13.148 & 12.456 & 12.114 & 107.7375 & 69,84,35 \\
SDSS J141530.05+572428.7  &  ----  &  T3:  & 16.734 & 15.821 & 15.544 & 25.6 & 18,13,4 \\
SDSS J141659.78+500626.4  &  ----  &  L4  & 16.95 & 15.955 & 15.597 & 22.15 & 28,18,29 \\
2MASS J14182962-3538060  &  ----  &  L1.5  & 15.165 & 14.253 & 13.691 & 28.210797 & 47,47,35 \\
2MASS J14192618+5919047  &  ----  &  L1:  & 16.507 & 15.69 & 15.26 &  ----  & 47,47 \\
SDSS J142227.25+221557.1  &  ----  &  L6.5::  & 17.064 & 16.032 & 15.642 &  ----  & 18,18 \\
2MASS J14283132+5923354  &  L4  &  L4.4  & 14.781 & 13.875 & 13.265 & 45.560281 & 68,3,13,35 \\
2MASS J14313097+1436539  &  L2  &  L3.5:  & 15.151 & 14.501 & 14.125 & 24.170048 & 80,71,71,35 \\
SDSS J143553.25+112948.6  &  ----  &  T2:  & 17.137 & 16.15 & 16.906 & 36.4 & 18,18,4 \\
SDSS J143945.86+304220.6  &  ----  &  T2.5  & 17.223 & 16.28 & 15.881 &  ----  & 18,18 \\
2MASS J14403186-1303263  &  L1  &  L1pec(sl. blue)  & 15.38 & 14.747 & 14.243 & 19.450801 & 47,47,47,35 \\
2MASSW J1439284+192915  &  L1  &  ----  & 12.759 & 12.041 & 11.546 & 70.5551 & 48,14,35 \\
2MASSW J1448256+103159  &  L4:  &  L4.7 FLD-G  & 14.556 & 13.433 & 12.683 & 69.635165 & 68,31,13,35 \\
Gliese 570D (J14571496-2121477)  &  T7  &  T7.5  & 15.324 & 15.268 & 15.242 & 169.3 & 8,9,14,29 \\
2MASS J15031961+2525196  &  T6  &  T5  & 13.937 & 13.856 & 13.963 & 155.77583 & 8,9,14,35 \\
2MASSW J1506544+132106  &  L3  &  L4  & 13.365 & 12.38 & 11.741 & 85.42498 & 39,13,17,35 \\
2MASSW J1507476-162738  &  L5  &  L5.5  & 12.83 & 11.895 & 11.312 & 134.947402 & 44,50,17,35 \\
SDSS J151114.66+060742.9  &  ----  &  T2  & 16.016 & 14.955 & 14.544 & 36.7 & 1,13,29 \\
2MASSW J1515008+484742  &  L6  &  L6  & 14.111 & 13.099 & 12.5 & 104.5 & 21,79,13,4 \\
SDSS J151506.11+443648.3  &  ----  &  L7.5:  & 16.583 & 15.636 & 14.757 & 27.8 & 18,13,4 \\
SDSS J151643.01+305344.4  &  ----  &  T0.5:  & 16.848 & 15.868 & 15.081 & 48.2 & 18,13,4 \\
SDSS J151603.03+025928.9  &  ----  &  T0:  & 17.23 & 15.997 & 15.433 &  ----  & 9,13 \\
2MASS J15200224-4422419A  &  L1  &  L2.5  & 13.55 & 12.73 & 12.27 & 54.5433 & 65,10,17,35 \\
SDSS J152039.82+354619.8  &  ----  &  T0:  & 15.54 & 14.579 & 14 & 57.4 & 18,13,4 \\
SDSS J152103.24+013142.7  &  ----  &  T3  & 16.399 & 15.576 & 15.347 & 43.3 & 62,13,4 \\
2MASS J15200224-4422419B  &  ----  &  L4.5  & 14.7 & 13.7 & 13.22 & 54.1903 & 17,17,35 \\
Gl 584C (J15232263+3014562)  &  L8  &  L8  & 16.056 & 14.928 & 14.348 & 53.7 & 44,37,13,29 \\
2MASSI J1526140+204341  &  L7  &  L5.5  & 15.586 & 14.497 & 13.922 & 48.313227 & 44,13,14,35 \\
2MASS J15293306+6730215  &  ----  &  L0:  & 16.327 & 15.34 & 14.722 & 13.507849 & 47,47,35 \\
SDSS J153417.05+161546.1AB  &  ----  &  T3.5  & 16.753 & 16.078 & 16.411 & 24.9 & 18,18,26 \\
2MASSI J1534498-295227  &  T6  &  T5.5  & 14.9 & 14.866 & 14.843 & 63 & 8,9,13,27 \\
SDSS J153453.33+121949.2  &  ----  &  L4:  & 15.332 & 14.303 & 13.827 & 50.082653 & 18,18,35 \\
SDSS J154009.36+374230.3  &  ----  &  L9:  & 16.558 & 15.348 & 14.739 & 40.8 & 18,13,4 \\
2MASS J15461461+4932114  &  ----  &  T2.5:  & 15.902 & 15.135 & 14.9 & 46.5 & 64,13,4 \\
2MASS J15462718-3325111  &  ----  &  T5.5  & 15.631 & 15.446 & 15.485 & 88 & 9,15,29 \\
SDSS J154849.02+172235.4  &  ----  &  L5  & 16.104 & 15.142 & 14.456 &  ----  & 18,18 \\
2MASS J15500845+1455180A  &  L3  &  ----  & 14.776 & 13.795 & 13.261 & 24.7 & 12,12,4 \\
2MASSI J1553022+153236  &  ----  &  T7  & 15.825 & 15.939 & 15.507 & 75.1 & 9,13,26 \\
2MASS J16150413+1340079  &  ----  &  T6  & 16.35 & 16.489 & 15.85 & 68.6 & 56,56,29 \\
SDSS J161731.65+401859.7  &  ----  &  L4  & 16.741 & 15.605 & 14.754 &  ----  & 18,18 \\
SDSS J162255.27+115924.1  &  ----  &  L6:  & 16.879 & 16.149 & 15.548 &  ----  & 18,18 \\
SDSSp J162414.37+002915.6  &  T6  &  T6  & 15.494 & 15.524 & 15.518 & 90.91 & 66,9,14,75 \\
SDSS J163030.53+434404.0  &  ----  &  L7:  & 16.634 & 15.438 & 14.652 & 44.7 & 50,13,4 \\
2MASSW J1632291+190441  &  L8  &  L8  & 15.867 & 14.612 & 14.003 & 65.79 & 48,9,17,25 \\
SDSS J163239.34+415004.3  &  ----  &  T1:  & 17.078 & 16.114 & 15.748 &  ----  & 9,13 \\
SDSS J163359.23-064056.5  &  ----  &  L6  & 16.138 & 15.165 & 14.544 & 35.67 & 18,18,74 \\
2MASS J16382073+1327354  &  ----  &  L2  & 16.452 & 15.447 & 14.961 &  ----  & 47,47 \\
2MASS J16452207+3004071  &  L3  &  L3.0  & 15.19 & 14.213 & 13.587 & 36.327352 & 21,3,13,35 \\
2MASSW J1645221-131951  &  L1.5  &  ----  & 12.451 & 11.685 & 11.145 & 88.697007 & 41,15,35 \\
SDSS J164916.89+464340.0  &  ----  &  L5  & 18.265 & 16.311 & 16.177 &  ----  & 18,18 \\
SDSS J165329.69+623136.5  &  L3  &  L1  & 15.089 & 14.442 & 14.069 & 26.214956 & 42,13,13,35 \\
DENIS-P J170548.38-051645.7  &  L0.5  &  L1:FLD-G  & 13.309 & 12.552 & 12.032 & 53.122037 & 68,2,13,35 \\
2MASS J17072343-0558249B  &  ----  &  L3  & 13.96 & 12.72 & 12.2 &  & 68,63 \\
2MASS J17111353+2326333  &  L0 gamma  &  L1:INT-G  & 14.499 & 13.668 & 13.056 & 30.866673 & 31,2,18,35 \\
2MASSI J1711457+223204  &  L6.5  &  L9::  & 17.089 & 15.797 & 14.727 & 33.11 & 44,13,13,77 \\
2MASSW J1728114+394859  &  L7  &  ----  & 15.988 & 14.756 & 13.909 & 36.4 & 44,16,27 \\
SDSS J173101.41+531047.9  &  ----  &  L6:  & 16.374 & 15.484 & 14.854 &  ----  & 18,18 \\
2MASS J17320014+2656228  &  ----  &  L1  & 15.931 & 15.018 & 14.461 & 16.834969 & 47,47,35 \\
2MASS J17392515+2454421  &  ----  &  L4  & 15.802 & 14.647 & 13.946 & 41.866723 & 47,47,35 \\
2MASS J17461199+5034036  &  L5  &  L5.7  & 15.096 & 14.047 & 13.529 & 48.34364 & 68,3,13,35 \\
2MASS J17502484-0016151  &  L5  &  L5.5  & 13.294 & 12.411 & 11.849 & 108.267596 & 66,43,13,34 \\
SDSSp J175032.96+175903.9  &  T4  &  T3.5  & 16.34 & 15.952 & 15.478 & 44.5 & 66,9,14,4 \\
2MASS J1754544+164920  &  ----  &  T5  & 15.762 & 15.531 & 14.788 & 64.3 & 85,85,4 \\
2MASS J17561080+2815238  &  sdL1  &  L1pec (blue)  & 14.712 & 14.135 & 13.813 & 28.93793 & 47,47,47,35 \\
SDSS J175805.46+463311.9  &  ----  &  T6.5  & 16.152 & 16.254 & 15.465 & 73.75 & 9,9,29 \\
2MASSI J1807159+501531  &  L1.5  &  L1  & 12.934 & 12.127 & 11.602 & 68.465705 & 20,79,15,35 \\
2MASS J18131803+5101246  &  ----  &  L5  & 15.915 & 15.11 & 14.432 &  ----  & 47,47 \\
2MASS J18212815+1414010  &  L4.5 pec  &  L5.5  & 13.431 & 12.396 & 11.65 & 107.0339 & 57,60,56,35 \\
2MASS J18283572-4849046  &  ----  &  T5.5  & 15.175 & 14.908 & 15.181 & 87.9 & 9,14,73 \\
2MASS J19010601+4718136  &  ----  &  T5  & 15.856 & 15.468 & 15.641 & 54.5 & 9,14,4 \\
2MASS J19163888-3700026  &  ----  &  L1  & 15.669 & 14.878 & 14.381 & 19.9789 & 47,47,35 \\
2MASS J19285196-4356256  &  L4  &  L4 pec  & 15.199 & 14.127 & 13.457 & 34.976993 & 68,61,13,35 \\
2MASS J19415458+6826021  &  ----  &  L2  & 15.99 & 15.2 & 14.711 &  ----  & 47,47 \\
2MASS J19495702+6222440  &  L2 pec (blue)  &  L2 pec (sl. blue)  & 16.359 & 15.47 & 14.75 &  ----  & 47,47,47 \\
2MASS J20025073-0521524  &  L5 beta  &  L7  & 15.316 & 14.278 & 13.417 & 56.696365 & 31,61,15,35 \\
2MASS J20261584-2943124  &  L1:  &  ----  & 14.802 & 13.946 & 13.36 & 29.272426 & 21,38,35 \\
SDSS J202820.32+005226.5  &  L3  &  L2  & 14.298 & 13.377 & 12.793 & 29.565069 & 42,13,14,35 \\
2MASS J20343769+0827009  &  L1  &  L0.5  & 14.464 & 13.593 & 13.08 & 35.565904 & 70,13,13,35 \\
2MASS J20360316+1051295  &  L3  &  L3.5  & 13.95 & 13.018 & 12.447 & 41.045782 & 68,13,13,35 \\
SDSS J204317.69-155103.4  &  ----  &  L9  & 16.625 & 16.054 & 15.402 & 22.8 & 18,13,73 \\
SDSS J204749.61-071818.3  &  ----  &  T0:  & 16.946 & 15.909 & 14.99 & 33.2 & 9,13,73 \\
SDSS J205235.31-160929.8  &  ----  &  T1:  & 16.334 & 15.414 & 15.123 & 33.7 & 18,13,27 \\
2MASSI J2057540-025230  &  L1.5  &  L2: FLD-G  & 13.121 & 12.268 & 11.724 & 64.710178 & 20,2,15,35 \\
2MASSW J2101154+175658  &  L7.5  &  ----  & 16.853 & 15.861 & 14.892 & 30.14 & 44,13,29 \\
2MASSI J2104149-103736  &  L2.5  &  L2  & 13.841 & 12.975 & 12.369 & 58.018297 & 46,13,13,35 \\
2MASSI J2107316-030733  &  L0  &  ----  & 14.2 & 13.443 & 12.878 & 26.014087 & 20,14,35 \\
SDSS J212413.89+010000.3  &  ----  &  T5  & 16.031 & 16.183 & 16.144 & 57 & 9,18,4 \\
2MASS J21321145+1341584  &  L6  &  L5  & 15.795 & 14.604 & 13.839 & 35.6 & 21,13,72,27 \\
2MASSW J2130446-084520  &  L1.5  &  M8.3  & 14.137 & 13.334 & 12.815 & 37.473873 & 46,3,47,35 \\
SDSS J213154.43-011939.3  &  L9:  &  L9  & 17.396 & 15.781 & 15.559 &  ----  & 36,18,18 \\
SDSS J213240.36+102949.4  &  ----  &  L2.0 FLD-G  & 16.594 & 15.366 & 14.634 &  ----  & 33,18 \\
SDSS J213352.72+101841.0  &  ----  &  L5:  & 16.878 & 15.833 & 15.236 &  ----  & 18,18 \\
2MASS J21392676+0220226  &  T2  &  T1.5  & 15.264 & 14.165 & 13.582 & 101.5 & 66,9,9,61 \\
2MASS J21420580-3101162  &  L3  &  L1.5 FLD-G  & 15.844 & 14.767 & 13.965 & 29.203964 & 52,33,13,35 \\
HN Peg B (J21442847+1446077)  &  ----  &  T2.5  & 16.7 & 15.55 & 15.63 & 54.37 & 59,59 \\
2MASS J21481628+4003593  &  L6  &  L6 FLD-G  & 14.147 & 12.783 & 11.765 & 123.675236 & 57,54,58,35 \\
2MASS J21512543-2441000  &  L3  &  L4 pec  & 15.752 & 14.571 & 13.649 &  ----  & 21,33,15 \\
2MASS J21513979+3402444  &  ----  &  L7 pec (sl. blue)  & 16.704 & 15.796 & 14.983 &  ----  & 47,47 \\
2MASS J21513839-4853542  &  ----  &  T4  & 15.73 & 15.168 & 15.431 & 60 & 9,9,73 \\
2MASS J21542494-1023022  &  ----  &  T4.5  & 16.425 & 16.454 & 17.045 & 37.2 & 56,56,73 \\
2MASS J21543318+5942187  &  ----  &  T5  & 15.661 & 15.765 & 15.338 & 64.7 & 56,56,5 \\
2MASS J21555848+2345307  &  ----  &  L2  & 15.986 & 14.951 & 14.268 &  ----  & 47,47 \\
2MASS J21580457-1550098  &  L4:  &  L5  & 15.04 & 13.867 & 13.185 & 43.109403 & 46,61,13,35 \\
DENIS-P J220002.05-303832.9B  &  L0  &  L0: FLD-G  & 14.36 & 13.57 & 13.09 & 25.459 & 68,55,6,35 \\
2MASS J22114470+6856262  &  ----  &  L2  & 15.712 & 14.813 & 14.185 & 25.062214 & 47,47,35 \\
2MASS J22120703+3430351  &  L5:  &  L6  & 16.316 & 15.182 & 14.37 &  ----  & 68,47,13 \\
2MASSW J2224438-015852  &  L4.5  &  L3:FLD-G  & 14.073 & 12.818 & 12.022 & 86.151353 & 44,55,13,35 \\
2MASS J22282889-4310262  &  ----  &  T6  & 15.662 & 15.363 & 15.296 & 92.1 & 9,14,61 \\
2MASS J22425317+2542573  &  L3  &  ----  & 14.812 & 13.744 & 13.048 & 46.938092 & 21,13,35 \\
2MASSW J2244316+204343  &  L6.5  &  L6:VL-G  & 16.476 & 14.999 & 14.022 & 58.7 & 46,2,58,55 \\
SDSSp J224953.45+004404.2  &  L4 gamma  &  L3:INT-G  & 16.587 & 15.421 & 14.358 & 25.5 & 30,2,15,55 \\
DENIS-P J225210.73-173013.4  &  ----  &  L7.5  & 14.313 & 13.36 & 12.901 & 60.578571 & 43,67,35 \\
2MASSI J2254188+312349  &  T5  &  T4  & 15.262 & 15.018 & 14.902 &  ----  & 66,9,14 \\
2MASS J23174712-4838501  &  L4  &  L6.5 pec (red)  & 15.15 & 13.925 & 13.181 & 49.962452 & 68,47,47,35 \\
2MASS J23254530+4251488  &  L8  &  L7.5:  & 15.493 & 14.452 & 13.764 & 69.228017 & 21,13,13,35 \\
2MASS J2325560-025950  &  L3:  &  ----  & 15.961 & 14.935 & 14.115 &  ----  & 13,13 \\
SDSS J232804.58-103845.7  &  ----  &  L3.5  & 17.005 & 15.841 & 15.083 &  ----  & 18,18 \\
2MASS J23312378-4718274  &  ----  &  T5  & 15.659 & 15.51 & 15.389 &  ----  & 9,14 \\
2MASS J23392527+3507165  &  L3.5  &  L3.0 FLD-G  & 15.362 & 14.351 & 13.588 & 36.230493 & 68,33,13,35 \\
2MASSI J2339101+135230  &  ----  &  T5  & 16.239 & 15.822 & 16.147 & 62.7 & 9,9,4 \\
2MASS J23512200+3010540  &  L5.5  &  L5: FLD-G  & 15.849 & 14.571 & 14.018 & 41.2 & 47,55,47,55 \\
2MASSI J2356547-155310  &  ----  &  T5.5  & 15.824 & 15.63 & 15.771 & 74.4 & 9,9,29 \\
\enddata

\tablecomments{List of all 301 archival spectra used in this project, along with their optical and infrared spectral types, 2MASS magnitudes, and parallaxes.}

\tablerefs{(1) \cite{Albert2011}; (2) \cite{Allers2013}; (3) \cite{Bard2014}; (4) \cite{Best2021}; (5) \cite{Best2021};(6) \cite{BurgMcel2006}; (7) \cite{Burg03_1086}; (8) \cite{Burg03_510}; (9) \cite{Burg06}; (10) \cite{Burg07}; (11) \cite{Burg08}; (12) \cite{Burg09}; (13) \cite{Burg10}; (14) \cite{Burg04}; (15) \cite{Burg08b}; (16) \cite{Burg2011}; (17) \cite{burg07b}; (18) \cite{Chiu06}; (19) \cite{cruz04}; (20) \cite{cruz03}; (21) \cite{cruz07}; (22) \cite{Cruz_2009}; (23) \cite{Cruz18}; (24) \cite{cush05}; (25) \cite{dahn02}; (26) \cite{dupuy12}; (27) \cite{dupuy17}; (28) \cite{fahe10}; (29) \cite{fahe12}; (30) \cite{fahe13}; (31) \cite{Faherty_2016}; (32) \cite{fan00}; (33) \cite{gagn15}; (34) \cite{gaia2description}, \cite{gaiaDR2}; (35) \cite{2021}; (36) \cite{gauz19}; (37) \cite{Geballe_2002}; (38) \cite{gel10}; (39) \cite{gizi00}; (40) \cite{gizis01}; (41) \cite{gizi02}; (42) \cite{hawley02}; (43) \cite{kend04}; (44) \cite{kirk00}; (45) \cite{kirk01}; (46) \cite{Kirkpatrick_2008}; (47) \cite{kirk10}; (48) \cite{Kirkpatrick_1999}; (49) \cite{Kirkpatrick_2006}; (50) \cite{knap04}; (51) \cite{lieb03}; (52) \cite{lieb06}; (53) \cite{lieb07}; (54) \cite{Liu13}; (55) \cite{liu16}; (56) \cite{looper07}; (57) \cite{looper08}; (58) \cite{looperetal08}; (59) \cite{luhman570}; (60) \cite{manj19}; (61) \cite{maro13}; (62) \cite{maro15}; (63) \cite{mcel06}; (64) \cite{metch08}; (65) \cite{phan08}; (66) \cite{pine16}; (67) \cite{reid06}; (68) \cite{reid08}; (69) \cite{schmidt10}; (70) \cite{schn2014}; (71) \cite{sheppard09}; (72) \cite{siegler07}; (73) \cite{smart13}; (74) \cite{smart18}; (75) \cite{tinney03}; (76) \cite{tinney14}; (77) \cite{vrba04}; (78) \cite{wilson01}; (79) \cite{wilson03}; (80) \cite{zhan09}; (81) \cite{stumpf09}; (82) \cite{bard19}; (83) \cite{scholz02}; (84) \cite{schmidtb}}

\end{deluxetable}

\end{document}
